Statistically Profiling Biases in Natural Language Reasoning Datasets and Models

Recent work has indicated that many natural language understanding and reasoning datasets contain statistical cues that may be taken advantaged of by NLP models whose capability may thus be grossly overestimated. To discover the potential weakness in the models, some human-designed stress tests have been proposed but they are expensive to create and do not generalize to arbitrary models. We propose a light-weight and general statistical profiling framework, ICQ (I-See-Cue), which automatically identifies possible biases in any multiple-choice NLU datasets without the need to create any additional test cases, and further evaluates through blackbox testing the extent to which models may exploit these biases.

==> demonstration.tex <==
\section{DEMONSTRATION}
\label{sec:demonstration}
% a simple tool for multiple choice dataset evaluation and correction
\subsection{Setup} 
We demonstrate our framework 
%with real-world and researchers can apply it to test 
%whether a test dataset is comprehensive or not 
%and evaluate a model from various aspects online.
%~\footnote{http://adapt.seiee.sjtu.edu.cn:3308/data\_traning/dataset}}, 
with 12 popular text inference datasets and 3 popular deep neural models.
The datasets can be 
classified into two types. 
The first type is NLI classification tasks (SNLI, QNLI, MNLI), 
a special case of multiple choice datasets. 
The second type is the multiple choice problems, 
%\KZ{Just call them MCQ? Is there a better name?} 
including ARCT, 
ARCT\_adv\cite{schuster2019towards}, 
RACE~\cite{lai2017race}, RECLOR~\cite{yu2020reclor}, 
%in which ``hypothesis'' 
%s one of the alternatives and ``premise'' contains more 
%than one context roles. 
Ubuntu~\cite{lowe2015ubuntu}, COPA~\cite{roemmele2011choice}, ROCStory, SWAG~\cite{zellers2018swag} and 
CQA~\cite{talmor2019commonsenseqa}.
%also belong to the second type but with only context role  in ``premise''. 
The models are fastText~\cite{joulin2017bag}, ESIM and Bert (base).
We set $k = 10$, which means for Word feature, we only consider 
top 10 words with highest feature score. 
The threshold $\sigma$ is set to 5. 

With our framework, we can find some features which influence the 
three models. Some examples are shown in \secref{sec:model}. 
User can try other features or even upload their own dataset or their own
model (in the form of a prediction result file). 
Special care should be taken when using the Word feature. 
If the frequency of a word is too low, there will be very few cases 
for testing this feature. We considered this 
problem and experimented with different thresholds and 
concluded that a word with frequency greater than 100 in the training data
will qualify as a feature. 

\subsection{Scenarios}
The demo will showcase the following scenarios.

\subsubsection{Dataset Evaluation}

\begin{figure}[th]
\centering
\includegraphics[width=1.0\columnwidth]{picture/dataset.jpg}
\caption{Web UI of ICQ}
\label{fig:dataset}
\end{figure}

%\KZ{The following needs to be rewritten as the fig is updated.}
We invite the users to experience interactive user interface of our 
framework (see \figref{fig:dataset}). 
In the ``Evaluate Dataset'' section,
users are able to upload their own dataset or select data sources we provide. 
User can also choose the features of interest to test.
In the result panel, users can view the distribution of training and test data  
with a specific feature. 
%If the JSD score is low, it means this feature is a cue. 
%For example, in \figref{fig:dataset_result}, we can get to know the distribution of 
%each word feature and the similarity between train and test data on this feature with 
%JSD score.



\subsubsection{Model Evaluation}
%\KZ{The following needs to be rewritten.}
%Over the features which have adequate samples, 
We also invite the users to 
submit a prediction result file of their model to view which features the 
model is sensitive to on ``Web UI of ICQ'' (see~\figref{fig:dataset}). 
In addition, we provide 3 models for our dataset as demo for users 
to test.  Using result panel, users can view the distribution of training dataset, 
even-out feature dataset and prediction result of a feature. The JSD score is 
calculated between training data distribution and predicting distribution.
% For example in 
%\figref{fig:model_result}, we can find that the Word features are less than before. 
%Because we only retain the feature which we have enough test samples with threshold 
%$\sigma$.

%\section{Result}


%We proceed to demonstrate the effectiveness of our framework in two aspects:
%First, 
%we use our method to detect cues and measure the amount of information leak
%in 12 datasets from 6 different tasks, as shown in~\tabref{tab:datasets_exp}. 
%Second, we evaluate the true reasoning power of a number of popular NLP
%models on original test sets that are split into 
%easy and hard part. 

%\begin{table*}[th]
%\centering:
%\includegraphics[width=2\columnwidth]{picture/datasets_exp.eps}
%\caption{Data examples and normalized version.}
%\label{tab:datasets_exp}
%\end{table*}
%
% \subsection{Our Results on Different Tasks}
% \label{sec:experiment1}
% 
% We experiment on 12 datasets in \tabref{tab:datasets_exp}. 
% %These datasets are widely used in their 
% %respective fields to provide relevant knowledge and evaluate whether 
%% models have the ability to solve the the problems in a field. %
%%We have give some examples in \figref{fig:datasets_exp}. 
%These datasets can mainly be classified into two types of tasks. 
%The first type are the NLI classification tasks, a special case of multiple choice datasets. 
%The second type are the multiple choice problems, including ARCT, 
%ARCT\_adv\cite{schuster2019towards}, 
%RACE~\cite{lai2017race}, and RECLOR~\cite{yu2020reclor}, in which ``hypothesis'' 
%is one of the alternatives and ``premise'' contains more than one context roles. 
%%\KZ{Don't understand: only has the premise and the hypothesis without the choices.}
%For example, in~\tabref{tab:datasets_exp}, 
%ARCT dataset have \textbf{Reason} and \textbf{Claim} as ``premise'' 
%which requires to select the right warrant between them. 
%%The alternative warrant is the hypothesis and the premise is consist of  reason and claim. 
%%RACE and Reclor includes context and questions which will be seen as ``premise''. 
%%The label for each alternative is 
%%``true'' or ``false'' for whether this hypothesis is the correct one.
%Ubuntu~\cite{lowe2015ubuntu}, COPA~\cite{roemmele2011choice}, ROCStory, SWAG~\cite{zellers2018swag} and 
%CQA~\cite{talmor2019commonsenseqa} also belong to the second type but with only context role 
%in ``premise''.
%
%To show if the word cues really exist in these datasets, 
%we use diverse metrics (in~\secref{sec:approach}) to get cue features. 
%Then we use four simplest ways, the average value classifier (Ave), 
%the maximum value classifier (Max), SGD classifier (SGDC) and 
%logistic regression (LR) (\secref{sec:approach}), 
%to make decision using only the spurious statistical cues. 
%
%
%In order to measure the severity of information leak in data sets, we propose to 
%use the deviation of accuracy from the majority prediction as a measurement which can be expressed as:
%\begin{equation}
%    \mathcal{D} = {Acc} - {Majority}
%\end{equation}
%
%${Majority}$ is the accuracy with majority voting. When the label distribution is balanced, the majority 
%voting is equal to random selection. ${Acc}$ represents the prediction result of 
%a model based on spurious cues only. 
%The difference between our method and the hypothesis-only method (which serves as
%the gold standard here) is that our method uses word-level cues that are interpretable,
%whereas the hypothesis-only method uses more complex cues extracted by advanced models
%which is not interpretable.
%
%
%To track the deviation performance $\mathcal{D}$ of hypothesis-only models,
%we use Pearson Correlation Coefficient(PCC) score to estimate the correlation 
%of deviation results between our methods and hypothesis-only models.  
%We used all the combinations of 8 cue score metrics and 
%4 aggregation algorithms on 12 datasets. We get the 12 deviations of each methods,
%one for each dataset. 
%Meanwhile, we get hypothesis-only deviation results of fasttext and BERT. 
%%Then we calculate all Pearson score between each of our method and hypothesis-only 
%%results. 
%The correlation result is shown in~\tabref{best_method}. 
%We can find that CP cue score with logistic regression model scores 97.17\% 
%with fastText and 97.34\% with BERT which indicates its high correlation 
%with the golden standard hypothesis-only models. 
%Thus we choose CP with logistic regression method to evaluate all datasets in
%the remaining experiments. 
%To further illustrate this trend, we plot $\mathcal{D}$ for 
%our CP+LR method and 2 hypothesis-only models (fastText and BERT) on 12 datasets
%in \figref{fig:d_figure}. 
%wE Can clearly see that the lines are tracking very closely.





==> system.tex <==
\section{system overview}
\label{sec:system}

\begin{figure}[th]
\centering
\includegraphics[width=1.0\columnwidth]{picture/framework.jpg}
\caption{Workflow}
\label{fig:framework}
\end{figure}

As illustrated in~\figref{fig:framework}, at the phase of data analysis, 
cue samples extraction, cue test data generation 
and distribution comparison, we can get to know 
whether the data have cue problem and analysis what features a model is really sensitive 
to in reasoning tasks.

%WeWe evaluate the information leak in the datasets by statistical cues only. 
%First, we formulate  a number of NL reasoning tasks in a general form. 
%Then based on the cues associated with each label, 
%we design a number of metrics to measure the correlation between words
%and labels. Such correlation scores are called ``cue scores'' because they are 
%indicative of potential cue patterns. Afterwards, we aggregate the scores using a number of simple statistical
%models to make the predictions. Finally, we show how to split a dataset into
%the easy and hard parts using the above fast predictions.

\subsection{Task Formulation}

%\textcolor{red}{Hongru: these are concrete examples, which i think should be given after the problem
%formulation} 
Given question instance $x$ of a natural language reasoning (NLR) task dataset $X$ 
we mentioned above, we formulate it as
\begin{equation}
    x = (p, h, l) \in X,
\end{equation}
\noindent
where $p$ is the context against which to do the reasoning, and $p$ corresponds 
to ``premise'' in~\exref{exp:snli};
$h$ is the hypothesis given the context $p$. $l \in \mathcal{L}$ is the label that 
depicts the type of relation between $p$ and $h$. 
The size of the relation set $\mathcal{L}$ varies between tasks. We argue that 
most of the discriminative NLR tasks can be formulated into this general form. 
%which will bring us much convenience to evaluate the cues of a dataset. 
For example, an NLI question consists of a \textit{premise}, a \textit{hypothesis} 
and a \textit{label} on the relation between premise and hypothesis. 
%The formulation of this task will be $p =$ \textit{premise}, $q =$ \textit{hypothesis} and $l =$ \textit{label}. 
$|\mathcal{L}| = 3$ for three different relations: 
\textit{entailment}, \textit{contradiction} and \textit{neutral}. 
We will talk about how to transform into this form in \secref{sec:dynamic}. 
%The ROCStory~\cite{mostafazadeh2016corpus} dataset
%such as in~\exref{exp:roc}, 
%consists of a \textbf{context} and two possible story \textbf{endings}. 

%We will formulate this task by setting $p = $ \textit{context}, $h = $ \textit{ending1/ending2}. In this case, $|\mathcal{L}| = 2$. because $l$ is ``true'' or ``false'' indicating whether 
%the ending is a plausible ending of the story.
\subsection{Analysis Data}


We need to analysis train dataset, test dataset and model prediction.

\subsection{Extract Samples Based on Features}
\label{sec:extract}

We suggest that users consider at least the following features: Word (unigram word in the task), 
Typos, NER (appropriately understanding named entities), 
Tense(understanding order of events), Negation, 
Sentiment, Overlap(overlap words between premise and hypothesis). 
This listing of cues is not exhaustive, but a starting point for users, 
who should also come up with additional features that are specific 
to their task or domain. We use $F$ to denote feature set.

\subsubsection{Word} For a dataset $X$, 
we collect a set of all words $\mathcal{N}$ that exist in $X$. 
%These 
%words can be word or cross-word that consists of a pair of
%unigrams, one from the premise and other from the hypothesis.
%the token pair between $p$ and $h$.
The feature metric for a word measures the disparity of the word's appearance under 
 a specific label. 
%The cross-unigrams, such as  ``swimmer-sea'' in~\exref{exp:snli}, 
%represent the 
%relational unigrams in a dataset. 
%The ``swimmer-sea'' cross-unigram can be identified as a cue if it always appear in the instances with 
%one label, like entailment.

Let $w$ be a word in $\mathcal{N}$, we compute a scalar statistic metric 
called {\em cue score}, $f^l$,  we use conditional probability(CP)
as the feature score to measure the correlation between words and labels 

\begin{equation}
    f^{(w,l)} = \frac{\#(w, l)}{\#(w)}
\end{equation}

We rank the words by feature score to $N^{'}$ and 
only treat top $k$ words as features:

\begin{equation}
    F_{W_i} = {w}_{i} , i \in 1...k \wedge w_{i} \in N^{'}
\end{equation}.
%of $w$ with respect to label $l$ as
%%\KZ{Consider changing $\mathcal{F}$ to $\mathcal{B}$ to avoid confusion with $f$?}
%
%\begin{equation}
%    f_{\mathcal{F}}^{l} = f_{\mathcal{F}}(w, l),    
%\end{equation}
%%We call $f_{\mathcal{F}}^{(k,l)}$ \textit{cue metric}, 
%where $f_{\mathcal{F}}^{l}$ is a function which measures how much spurious information can be conveyed by token $w_k$ for a particular label $l$. 
%$\mathcal{F}$ is a set of cue metrics that we used for computing the \textit{cue score}. 

\subsubsection{Sentiment}

We assigned sentiment features $F_{S}$as 
positive, negative, or neutral sentiment to each hypothesis which 
represented as: 
$S(h) = sign(number of positive words - number of negative words) in the hypothesis$.
The sentiment polarity of a word
is determined by a look-up from pre-trained
sentiment lexica\footnote{nltk}. 

\subsubsection{Tense}

Considering the order of events can is also an 
important information for commonsense reasoning, we include 
\textit{past}, \textit{present}, \textit{future} as Tense features $F_{Tense}$. 
The tense is determined by verb tags of dependency parsing~\footnote{scipy}.

\subsubsection{Negation}

Many work has observed that 
strong negation words (“no”, “not”) cause the model to predict contradiction for
neutral or entailed statements .Thus we think negation feature $F_{Neg}$can be a factor which affect models 
to make decisions. Negation is also decided on dependency parsing tags.

\subsubsection{Overlap}

In many cases, large word-overlap between premise and hypothesis sentences causes
wrong entailment prediction, even if they are unrelated. 
Very little word overlap causes a prediction
of neutral instead of entailment. Thus we wonder to 
know whether overlap feature $F_{O}$ can 
really influence models.

\subsubsection{NER}

The failure for the NER tests in CheckList~\cite{}
indicates that these models are relying on shortcuts
such as anchoring on named entities too strongly
instead of understanding named entities and their
impact on whether questions are duplicates. We also 
take in NER feature $F_{NER}$ in our feature test.

\subsubsection{Typos}

The premise or the hypothesis is ill-formed because of spelling errors. 
Typo feature $F_{Typos}$ many also can be learned by models as off-site information. 
We use a pretrained spelling model to get the typo information in a 
sentence. 

Given the features $F$, we can extract samples which contain a specific 
feature for training dataset and test dataset. In~\figref{fig:framework}, the blue 
distribution and red distribution represent  train and test data distribution based on 
a certain feature. We use mean square deviation(MSD) to measure the balance rate 
of a feature in a dataset. Then, we can observe which feature of the test set 
is insufficient for testing if the filtered test data size is quite small or samples on 
some label is rare which bellow a threshold $\sigma$. 
We can point out what kind of test samples should be augmented. 
but don't provide new method for data augmentation. 
%We only pay attention to the features which have enough test data for model evaluation.
%In addition, we can analysis the credibility of test data through 
%the Kullback-Leibler (KL) Divergence. If a train dataset distribution is unbalance, 
%a similar distribution between train and T
%test can lead to insufficient test which test the cues mostly with a certain label. 


\subsection{Generate stress test data}
\label{sec:generate}

We require a more fair dataset to test if a model is sensitive to a feature.
The extracted test dataset in \figref{fig:framework} (red) is unbalance with 
labels. Thus We assign a threshold for the smallest in test samples 
organized by different labels to decide whether this feature can be well tested 
with filtered dataset. If the test samples are adequate, we even-out the samples 
with various labels just as the yellow part in \figref{fig:framework}. Then we test the model 
on the reconstructed feature test data, the similarity between prediction result (green) and 
training data distribution(blue) on a feature indicates how the model is influenced by 
the appearance of the feature in training data. The similarity is 
calculated by Kullback-Leibler (KL) Divergence.

\subsection{Transformation of MCQs with dynamic choices}
\label{sec:dynamic}
So far the multiple-choice questions we targeted such as NLI problems
are actually classification problems with fixed set of choices. There is
another type of language reasoning tasks which are also in the form of
multiple-choice questions, but their choices are not fixed, as shown
below. 
\begin{example}\label{exp:roc}
An example question in ROCStory~\cite{mostafazadeh2016corpus}.\\
\noindent
\textbf{Context}: Rick grew up in a troubled household. 
He never found good support in family, and turned to gangs.           
It was n't long before Rick got shot in a robbery.             
The incident caused him to turn a new leaf.\\
\noindent
\textbf{Ending 1}: He joined a gang. \\
\noindent
\textbf{Ending 2}:  He is happy now.\\
\noindent
\textbf{Answer}: 2
\end{example}

In this type of tasks,
we can separate the original story into two unified instances, 
$u_1=(context, ending1, false)$ and $u_2=(context, ending2, true)$.
We can predict the label with probability for each instance $\mathcal{G}(input(u_1);\phi)$ and 
 $\mathcal{G}(input(u_2);\phi)$.
Then we can choose the ending with higher probability to make the prediction.
%For better take advantage of the bias score to choose the right choice. We also use two linear model: SGDClassifier and 
%logistic regression. The inputs of the models for instance $e_n$ is the concatenation of bias scores for each label which %can express as :  $input(e_n) = [ f_{\mathcal{F}}^{(w_{n_1}^{l_1})},..., f_{\mathcal{F}}^{(w_{n_d}^{l_1})},..., f_{\mathcal{F}}^{(w_{n_1}^{l_v})},..., f_{\mathcal{F}}^{(w_{n_d}^{l_v})}]$. The corresponding target is the correct label $l_{gold}\in{L}$.

 


